Limits of constant-parameter constitutive models for hydrogels under inertial cavitation

Mechanical characterization of soft materials at high strain rates is challenging due to their high compliance, nonlinear viscoelastic behavior, and potentially history-dependent responses. Inertial microcavitation rheometry (IMR) addresses this challenge by coupling laser-induced cavitation (LIC) experiments with numerical simulations of bubble dynamics models to infer constitutive models and material parameters. Both IMR and its variants infer parameters that depend on the chosen fitting window, which suggests that a constant-parameter constitutive model is insufficient to describe the full cavitation event. We use this window dependence to identify when the constant-parameter assumption fails, rather than to report a single effective parameter set. The constitutive parameters are estimated over moving, overlapping windows using a modified iterative ensemble Kalman smoother with multiple data assimilation (MIEnKS-MDA). Within the neo-Hookean Kelvin--Voigt (NHKV) constitutive model, we obtain time-resolved estimates of the constitutive response in polyacrylamide (PAAm) hydrogels with different crosslinker concentrations. The inferred shear modulus and viscosity generally decrease and then plateau during cavitation, while exhibiting relatively weak temperature sensitivity. For gelatin gels, by contrast, the inferred property evolution shows a pronounced temperature dependence, with distinct trends at low and high temperatures. Moreover, both the apparent shear modulus and viscosity exhibit significant variations during the first two bubble collapses. These results show that time-resolved parameter estimation within the prescribed NHKV constitutive structure can diagnose where the constant-parameter model assumption falls short during cavitation, thereby guiding the development of improved physics-based models of complex bubble--material interactions.

==> colors.tex <==
\definecolor{lightblue}{rgb}{0.63, 0.74, 0.78}
\definecolor{seagreen}{rgb}{0.18, 0.42, 0.41}
\definecolor{orange}{rgb}{0.85, 0.55, 0.13}
\definecolor{silver}{rgb}{0.69, 0.67, 0.66}
\definecolor{rust}{rgb}{0.72, 0.26, 0.06}
\definecolor{purp}{RGB}{68, 14, 156}

\colorlet{lightrust}{rust!50!white}
\colorlet{lightorange}{orange!25!white}
\colorlet{lightlightblue}{lightblue}
\colorlet{lightsilver}{silver!30!white}
\colorlet{darkorange}{orange!75!black}
\colorlet{darksilver}{silver!65!black}
\colorlet{darklightblue}{lightblue!65!black}
\colorlet{darkrust}{rust!85!black}
\colorlet{darkseagreen}{seagreen!85!black}

==> mathsymbols.tex <==
\usepackage{bm}
\newcommand{\ve}[1]{\bm{#1}}

\newcommand{\ba}{\ve{a}}
\newcommand{\bb}{\ve{b}}
\newcommand{\bu}{\ve{u}}
\newcommand{\bv}{\ve{v}}
\newcommand{\br}{\ve{r}}
\newcommand{\bp}{\ve{p}}
\newcommand{\bt}{\ve{t}}
\newcommand{\bn}{\ve{n}}
\newcommand{\bc}{\ve{c}}
\newcommand{\bq}{\ve{q}}
\newcommand{\bff}{\ve{f}}
\newcommand{\bw}{\ve{w}}
\newcommand{\by}{\ve{y}}
\newcommand{\bx}{\ve{x}}
\newcommand{\be}{\ve{e}}
\newcommand{\bg}{\ve{g}}
\newcommand{\bh}{\ve{h}}
\newcommand{\bs}{\ve{s}}
\newcommand{\bk}{\ve{k}}

\newcommand{\bA}{\ve{A}}
\newcommand{\bD}{\ve{D}}
\newcommand{\bJ}{\ve{J}}
\newcommand{\bS}{\ve{S}}
\newcommand{\bB}{\ve{B}}
\newcommand{\bU}{\ve{U}}
\newcommand{\bV}{\ve{V}}
\newcommand{\bW}{\ve{W}}
\newcommand{\bE}{\ve{E}}
\newcommand{\bQ}{\ve{Q}}
\newcommand{\bP}{\ve{P}}
\newcommand{\bGG}{\ve{G}}
\newcommand{\bRR}{\ve{R}}
\newcommand{\bX}{\ve{X}}
\newcommand{\bM}{\ve{M}}
\newcommand{\bC}{\ve{C}}
\newcommand{\bF}{\ve{F}}
\newcommand{\bI}{\ve{I}}
\newcommand{\bL}{\ve{L}}
\newcommand{\bR}{\ve{R}}

\newcommand{\tn}{\tilde{n}}

\newcommand{\cM}{\mathcal{M}}

\newcommand{\dd}{\text{d}}
\newcommand{\ddd}{\dd R \dd \dot{R}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\Rdot}{\dot{R}}
\newcommand{\Rddot}{\ddot{R}}

\newcommand{\muR}{\mu_R}
\newcommand{\muRdot}{\mu_{\dot{R}}}
\newcommand{\sigmaR}{\sigma_R}
\newcommand{\sigmaRdot}{\sigma_{\dot{R}}}

\newcommand{\bmu}{\vec{\boldsymbol{\mu}}}
\newcommand{\btheta}{\vec{\boldsymbol{\theta}}}

\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bEps}{\boldsymbol{\varepsilon}}
\newcommand{\beps}{\boldsymbol{\varepsilon}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\heps}{\hat{\varepsilon}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\vblambda}{\vec{\boldsymbol{\lambda}}}
\newcommand{\vbsigma}{\vec{\boldsymbol{\sigma}}}
\newcommand{\vbEps}{\vec{\boldsymbol{\varepsilon}}}
\newcommand{\vbdelta}{\vec{\boldsymbol{\delta}}}
\newcommand{\eps}{\varepsilon}

\newcommand{\vq}{\vec{q}}

\newcommand{\vba}{\vec{\ve{a}}}
\newcommand{\vbu}{\vec{\ve{u}}}
\newcommand{\vbx}{\vec{\ve{x}}}
\newcommand{\vby}{\vec{\ve{y}}}
\newcommand{\vbm}{\vec{\ve{M}}}
\newcommand{\vbmm}{\vec{\ve{m}}}
\newcommand{\vbv}{\vec{\ve{v}}}
\newcommand{\vbh}{\vec{\ve{h}}}
\newcommand{\vbbh}{\vec{\bar{\ve{h}}}}
\newcommand{\vbs}{\vec{\ve{s}}}
\newcommand{\vbF}{\vec{\ve{F}}}
\newcommand{\vbg}{\vec{\ve{g}}}
\newcommand{\vbq}{\vec{\ve{q}}}
\newcommand{\vbr}{\vec{\ve{r}}}

\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}

\newcommand{\hbx}{\hat{\ve{x}}}
\newcommand{\hby}{\hat{\ve{y}}}
\newcommand{\hbz}{\hat{\ve{z}}}

\newcommand{\hbF}{\widehat{\ve{F}}}
\newcommand{\hbq}{\widehat{\ve{q}}}
\newcommand{\hbg}{\widehat{\ve{g}}}
\newcommand{\hw}{\widehat{w}}

\newcommand{\hR}{\widehat{R}}
\newcommand{\hRdot}{\widehat{\dot{R}}}

\newcommand{\trho}{\widetilde{\rho}}
\newcommand{\tbrho}{\widetilde{\boldsymbol{\rho}}}
\newcommand{\tx}{\widetilde{x}}
\newcommand{\tbx}{\widetilde{\ve{x}}}
\newcommand{\tbB}{\widetilde{\ve{B}}}

\newcommand{\mom}{\mu}
\newcommand{\bmom}{\boldsymbol{\mu}}
\newcommand{\vbmom}{\vec{\bmom}}
\newcommand{\hbmom}{\widehat{\bmom}}


\newcommand{\EV}{\mathbb{E}}

\newcommand{\dt}{\Delta \tau}
\newcommand{\gdot}{\dot\gamma}

\newcommand\Rey{\mbox{\text{Re}}\xspace}

\newcommand{\cD}{\mathcal{D}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\dL}{\mathbf{L}}
\newcommand{\dW}{\mathbf{W}}
\newcommand{\dO}{\mathbf{O}}
\newcommand{\dM}{\mathbf{M}}
\newcommand{\dU}{\mathbf{U}}
\newcommand{\dD}{\mathbf{D}}

\newcommand{\cbL}{\overline{\mathcal{L}}}
\newcommand{\baru}{\bar{u}}
\newcommand{\barc}{\bar{c}}
\newcommand{\bars}{\bar{s}}

\newcommand{\bbarf}{\bar{\ve{f}}}
\newcommand{\barbu}{\bar{\ve{u}}}
\newcommand{\transpose}{\mathsf{T}}

==> preamble.tex <==
\makeatletter
  \long\def\pprintMaketitle{\clearpage
  \iflongmktitle\if@twocolumn\let\columnwidth=\textwidth\fi\fi
  \resetTitleCounters
  \def\baselinestretch{1}%
  \printFirstPageNotes
  \begin{center}%
 \thispagestyle{pprintTitle}%
   \def\baselinestretch{1}%
    {\large\bf\@title}\par\vskip5pt
    \normalsize\elsauthors\par\vskip5pt
    \footnotesize\itshape\elsaddress\par\vskip10pt
    % \hrule\vskip12pt
    % \ifvoid\absbox\else\unvbox\absbox\par\vskip10pt\fi
    % \ifvoid\keybox\else\unvbox\keybox\par\vskip10pt\fi
    % \hrule\vskip12pt
    \end{center}%
  \gdef\thefootnote{\arabic{footnote}}%
  }
\makeatother

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
% \journal{}

\raggedbottom
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{lipsum}
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{epsf}
\usepackage{setspace}
\usepackage{float}
\usepackage{soul}
\setstcolor{red}
% \usepackage[mediumspace,mediumqspace,squaren]{SIunits}

\usepackage[]{siunitx}
\sisetup{separate-uncertainty = true,print-unity-mantissa=false,per-mode=symbol,range-phrase = \text{--},range-units=single}

\usepackage[]{microtype}
\SetTracking{encoding={*}, shape=sc}{40}

\usepackage[margin=1in]{geometry}
\usepackage{abstract}
\usepackage{booktabs}

\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}

\usepackage[]{xcolor}
% \input{mathsymbols.tex}
\input{colors.tex}

\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
}

\usepackage{etoolbox}
\AtBeginEnvironment{tabular}{\small}

\usepackage[labelfont=bf,font=small]{caption}

\setlength{\parskip}{5pt}
\setlength{\parindent}{0pt}

\usepackage[nameinlink]{cleveref}
\crefname{equation}{}{}

\usepackage[parfill]{parskip}

\newcommand{\spencer}[1]{\textcolor{seagreen}{[[Spencer says: #1]]}}
\newcommand{\jbe}[1]{\textcolor{darklightblue}{[[JE: #1]]}}
\newcommand{\Red}[1]{{\color{red}#1}}
% \todo is redefined after \usepackage{changes} below (changes also defines \todo)

\usepackage{physics}
\AtBeginDocument{\RenewCommandCopy\qty\SI}

\usepackage{multirow}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{changes}
\renewcommand{\todo}[1]{{\color{red}[[TODO: #1]]}}
\newcommand{\suggestion}[1]{{\color{darkseagreen}[[FIX: #1]]}}

\makeatletter
\renewcommand{\Function}[2]{%
  \csname ALG@cmd@\ALG@L @Function\endcsname{#1}{#2}%
  \def\jayden@currentfunction{#1}%
}
\newcommand{\funclabel}[1]{%
  \@bsphack
  \protected@write\@auxout{}{%
    \string\newlabel{#1}{{\jayden@currentfunction}{\thepage}}%
  }%
  \@esphack
}

\newcommand{\mF}{\mathcal{F}}
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mM}{\mathcal{M}}

\newcommand{\btQ}{\vb*{\tilde{Q}}}
\newcommand{\btY}{\vb*{\tilde{Y}}}
\newcommand{\bcY}{\vb*{\check{Y}}}
\DeclareMathOperator*{\argmax}{arg\!\max}
\DeclareMathOperator*{\argmin}{arg\!\min}
\newcommand{\transpose}{\mathsf{T}}

\usepackage{mathtools}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\infdiv}{D_{\mathrm{KL}}\infdivx}
\DeclareSIUnit{\fps}{fps}

% Line numbers for peer review (with amsmath display-math patch)

\makeatother

